System G Distributed Graph Database

Motivated by the need to extract knowledge and value from interconnected data, graph analytics on big data is a very active area of research in both industry and academia. To support graph analytics efficiently a large number of in memory graph libraries, graph processing systems and graph databases have emerged. Projects in each of these categories focus on particular aspects such as static versus dynamic graphs, off line versus on line processing, small versus large graphs, etc. While there has been much advance in graph processing in the past decades, there is still a need for a fast graph processing, using a cluster of machines with distributed storage. In this paper, we discuss a novel distributed graph database called System G designed for efficient graph data storage and processing on modern computing architectures. In particular we describe a single node graph database and a runtime and communication layer that allows us to compose a distributed graph database from multiple single node instances. From various industry requirements, we find that fast insertions and large volume concurrent queries are critical parts of the graph databases and we optimize our database for such features. We experimentally show the efficiency of System G for storing data and processing graph queries on state-of-the-art platforms.

==> data/vertex/junk.tex <==
   \iffalse
                \addplot [mark size=1pt, mark=o, color=blue] table [x=batch, y=rate]{data/vertex/plot_single.txt};
                \addplot [mark size=2pt, mark=otimes, color=orange] table [x=batch, y=rate]{data/vertex/plot_dist1.txt};
                \addplot [mark size=2pt, mark=square, color=red] table [x=batch, y=rate]{data/vertex/plot_dist12.txt};
                \addplot [mark size=2pt, mark=x, color=olivegreen] table [x=batch, y=rate]{data/vertex/plot_neo4j.txt};
                \addplot [mark size=2pt, mark=diamond, color=black] table [x=batch, y=rate]{data/vertex/plot_janus.txt};
                \legend{Single node, dist\_1shard, dist\_12shard, neo4j, Janus}
                \fi
                
                
                
                
                
 \begin{tikzpicture}
            \begin{axis}[
                    width=.95\linewidth,
                    height=.59\linewidth,
                    axis lines = left,              
                    xlabel={batch number},
                    xmin=0, xmax=50,
                    ymin=0, ymax=500000,
                    xtick = {},
                    ymajorgrids=true,
                    grid style=dashed,
                    ylabel={Insertion Rate (vertices/sec)},
                %    y label style={at={(axis description cs:.1,.5)},anchor=south},
                    %ytick = {0,1,2,3,4},
                    tick label style={font=\scriptsize},
                    legend style={font=\scriptsize, at={(0.45,0.5)}},
                   ]
             
                 \addplot table [x=batch, y=rate]{data/vertex/plot_single.txt};
                \addplot  table [x=batch, y=rate]{data/vertex/plot_dist1.txt};
               
                \addplot table [x=batch, y=rate]{data/vertex/plot_neo4j.txt};
                \addplot  table [x=batch, y=rate]{data/vertex/plot_janus.txt};
                \legend{Single node, dist\_1shard, dist\_12shard, neo4j, Janus}
                
            \end{axis}
        \end{tikzpicture}



 \begin{tikzpicture}
    \begin{axis}[
                    width=.95\linewidth,
                    height=.59\linewidth,
                    axis lines = left,              
                    xlabel={Num_threads},
                    xmin=0, xmax=4,
                    ymin=0, ymax=200,
                    xtick = data,
                    xticklabel={1,2,4,8}
                    ymajorgrids=true,
                    grid style=dashed,
                    ylabel={Query Time (Sec)},
                %    y label style={at={(axis description cs:.1,.5)},anchor=south},
                    %ytick = {0,1,2,3,4},
                    tick label style={font=\scriptsize},
                    legend style={font=\scriptsize, at={(0.45,0.5)}},
                   ]
                   
                \addplot [mark=diamond,color=BurntOrange]  table  [x=thread, y=time]{data/bfs/single.txt};
                \addplot [mark=x, color=olivegreen]  table [x=thread, y=time]{data/bfs/dist1.txt};
               \addplot [mark=o, color=blue]  table [x=thread, y=time]{data/bfs/dist12.txt};    
                \addplot [mark=square, color=gray] table [x=thread, y=time]{data/bfs/neo4j.txt};
                 
                \legend{SG-Single, SG-1shard, SG-12shard, neo4j}
    \end{axis}
\end{tikzpicture}
